A Novel a priori State Computation Strategy for the Unscented Kalman Filter to Improve Computational Efficiency

A priori state vector and error covariance computation for the Unscented Kalman Filter (UKF) is described. The original UKF propagates multiple sigma points to compute the a priori mean state vector and the error covariance, resulting in a higher computational time compared to the Extended Kalman Filter (EKF). In the proposed method, the posterior mean state vector is propagated and then the sigma points at the current time step are calculated using the first-order Taylor Series approximation. This reduces the computation time significantly, as demonstrated using two example applications which show improvements of 90.5% and 92.6%. This method shows the estimated state vector and the error covariance are accurate to the first-order Taylor series terms. A second method using Richardson Extrapolation improves prediction accuracy to the second-order Taylor series terms. This is implemented on the two examples, improving efficiency by 85.5% and 86.8%.

==> Analysis.tex <==
\subsection{Error Analysis}
In this section, the error incurred due to the approximation mentioned in \ref{sec:proposed_strategy} is assessed. Hereafter, the sigma points and mean calculates using the proposed approximation will be denoted as $\bf \widetilde{Y}_i$ and $\bf \widetilde{\overline{Y}}$. 

\subsection{Error in mean due to approximation}
Let ${\bf Y_i}(t)$ is propagated using numerical integration from the equation \ref{eq:propagation}. Then, from \ref{eq:sigmapt} and \ref{eq:sigma_approx} error due to approximation in each sigma point (neglecting the truncation and round off error) is
\begin{align}
{\bf Y_i}(t+\delta t) - {\bf \widetilde{Y}_i}(t+\delta t) &= \frac{{\bf D_{\Delta Y_i}^2 F}}{2!} +\frac{{\bf D_{\Delta Y_i}^3 F}}{3!}+....\nonumber\\
&= e_i
\label{eq:error_i}
\end{align} 
The mean state vector using the original Unscented transformation \cite{Julier2000}
\begin{align}
{\bf\overline{Y}}^-(t+\delta t) &= \frac{1}{n+\kappa}\left[\kappa{\bf Y_0}(t+\delta t) +\frac{1}{2}\sum_{i=1}^{2n}\left[{\bf Y_i}(t+\delta t)\right]\right]\nonumber\\
&={\bf Y_0}(t+\delta t) + \frac{1}{2(n+\kappa)}\sum_{i=1}^{2n}\left[{\bf D_{\Delta Y_i}F} + \frac{{\bf D_{\Delta Y_i}^2 F}}{2!} +\frac{{\bf D_{\Delta Y_i}^3 F}}{3!}+....\right]\label{eq:mean_UKF}
\end{align}
Similarly using the proposed approximation, the mean vector is
\begin{align}
{\bf\widetilde{\overline{Y}}}^-(t+\delta t) &= \frac{1}{n+\kappa}\left[\kappa{\bf Y_0}(t+\delta t) +\frac{1}{2}\sum_{i=1}^{2n}\left[{\bf \widetilde{Y}_i}(t+\delta t)\right]\right]\nonumber\\
&={\bf Y_0}(t+\delta t) + \frac{1}{2(n+\kappa)}\sum_{i=1}^{2n}{\bf D_{\Delta Y_i}F}\label{eq:approx_ukf}
\end{align}
The error in mean prediction due to the approximation is
\begin{align}
{\bf\overline{Y}}^-(t+\delta t)-{\bf\widetilde{\overline{Y}}}^-(t+\delta t)&= \frac{1}{2(n+\kappa)}\sum_{i=1}^{2n}\left[\frac{{\bf D_{\Delta Y_i}^2 F}}{2!} +\frac{{\bf D_{\Delta Y_i}^3 F}}{3!}+....\right]
\nonumber\\
&=\bar{e}\label{eq:mean_error}
\end{align}

\subsection{Error in covariance due to approximation}
Let us define the predicted covariance using the original Unscented transformation as \cite{Julier2000}
\begin{equation}
{\bf P^-_{YY}}(t+\delta t)=\frac{1}{n+\kappa}\left[\kappa\left[{\bf Y_0}-{\bf \overline{Y}^-}\right]\left[{\bf Y_0}-{\bf \overline{Y}^-}\right]^T+\frac{1}{2}\sum_{i=1}^{2n}\left[{\bf Y_i}-{\bf \overline{Y}^-}\right]\left[{\bf Y_i}-{\bf \overline{Y}^-}\right]^T\right]
\label{eq:cov}
\end{equation}
and the predicted covariance using the new approximation as
\begin{equation}
{\bf \widetilde{P}_{YY}}^-(t+\delta t)=\frac{1}{n+\kappa}\left[\kappa\left[{\bf Y_0}-{\bf \widetilde{\overline{Y}}^-}\right]\left[{\bf Y_0}-{\bf \widetilde{\overline{Y}}^-}\right]^T+\frac{1}{2}\sum_{i=1}^{2n}\left[{\bf \widetilde{Y}_i}-{\bf \widetilde{\overline{Y}}^-}\right]\left[{\bf \widetilde{Y}_i}-{\bf \widetilde{\overline{Y}}^-}\right]^T\right]
\label{eq:cov_aprx}
\end{equation}

Using equations \ref{eq:error_i}, \ref{eq:mean_error}, \ref{eq:cov} and \ref{eq:cov_aprx}, one can write,
\begin{align}
{\bf P^-_{YY}}(t+\delta t)=&{\bf \widetilde{P}_{YY}}^-(t+\delta t)+\frac{\kappa}{n+\kappa}\left[\bar{e}\bar{e}^T-\bar{e}\left[{\bf Y_0}-{\bf \widetilde{\overline{Y}}^-}\right]^T-\left[{\bf Y_0}-{\bf \widetilde{\overline{Y}}^-}\right]\bar{e}^T\right]\nonumber\\
&+\frac{1}{2(n+\kappa)}\sum_{i=1}^{2n}\left[[e_i-\bar{e}]\left[{\bf \widetilde{Y}_i}-{\bf \widetilde{\overline{Y}}^-}\right]^T+\left[{\bf \widetilde{Y}_i}-{\bf \widetilde{\overline{Y}}^-}\right][e_i-\bar{e}]^T+[e_i-\bar{e}][e_i-\bar{e}]^T\right]
\label{eq:cov_error}
\end{align}

==> EUKF_result.tex <==
%\subsection{State Estimation using Extrapolated Single Propagation Unscented Kalman Filter}
%\label{sec:EUKF}
\begin{figure}[h!]%
\centering
\includegraphics[width=\columnwidth]{prcsT_vs_error.jpg}%
\caption{Processing time vs. estimation error for different algorithms}%
\label{fig:comp_graph}%
\end{figure} 
It is observed that the ESPUKF provides lower altitude estimation error compared to the SPUKF. The altitude estimation error using the ESPUKF is comparable with the UKF and the SSUKF results. In table \ref{tab:EUKF}, processing time per time step and average altitude estimation error at steady state is shown. In figure \ref{fig:comp_graph} processing time vs. absolute average steady state estimation error is plotted. It is clear that ESPUKF provides the most desirable performance as compared to the other algorithms when processing time is a constraint.
